On C*-algebras of irreversible algebraic dynamical systems

Extending the work of Cuntz and Vershik, we develop a general notion of independence for commuting group endomorphisms. Based on this concept, we initiate the study of irreversible algebraic dynamical systems, which can be thought of as irreversible analogues of the dynamical systems considered by Schmidt. To each irreversible algebraic dynamical system, we associate a universal C*-algebra and show that it is a UCT Kirchberg algebra under natural assumptions. Moreover, we discuss the structure of the core subalgebra, which is closely related to generalised Bunce-Deddens algebras in the sense of Orfanos. We also construct discrete product systems of Hilbert bimodules for irreversible algebraic dynamical systems which allow us to view the associated C*-algebras as Cuntz-Nica-Pimsner algebras. Besides, we prove a decomposition theorem for semigroup crossed products of unital C*-algebras by semidirect products of discrete, left cancellative monoids.

==> bib.tex <==

%\begin{bibdiv}
\begin{biblist}

\bib{AD}{article}{%MR919508,
    AUTHOR = {Anantharaman-Delaroche, Claire},
     TITLE = {Syst\`{e}mes dynamiques non commutatifs et moyennabilit\'{e}},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {279},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {297--315},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L55 (22D25 22D40 43A07 43A35)},
 % MRNUMBER = {919508 (89f:46127)},
%MRREVIEWER = {Elliot C. Gootman},
       DOI = {\href{http://dx.doi.org/10.1007/BF01461725}{10.1007/BF01461725}},
}

\bib{AR}{incollection} {%MR1491110,
    AUTHOR = {Arzumanian, Victor},
    AUTHOR = {Renault, Jean},
     TITLE = {Examples of pseudogroups and their C*-algebras},
 BOOKTITLE = {Operator algebras and quantum field theory ({R}ome, 1996)},
     PAGES = {93--104},
 PUBLISHER = {Int. Press, Cambridge, MA},
      YEAR = {1997},
  % MRCLASS = {46L05},
 % MRNUMBER = {1491110 (99a:46101)},
%MRREVIEWER = {Siegfried Echterhoff},
}

\bib{AS}{article}{%MR1258035,
    AUTHOR = {Archbold, Robert J.},
    AUTHOR = {Spielberg, Jack S.},
     TITLE = {Topologically free actions and ideals in discrete C*-dynamical systems},
   JOURNAL = {Proc. Edinburgh Math. Soc. (2)},
 % FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {37},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {119--124},
      ISSN = {0013-0915},
%     CODEN = {PRMSA3},
 %  MRCLASS = {46L55},
  %MRNUMBER = {1258035 (94m:46101)},
%MRREVIEWER = {Yasuyuki Kawahigashi},
       DOI = {\href{http://dx.doi.org/10.1017/S0013091500018733}{10.1017/S0013091500018733}},
}

\bib{Bae}{article}{%MR0009955,
    AUTHOR = {Baer, Reinhold},
     TITLE = {Groups without proper isomorphic quotient groups},
   JOURNAL = {Bull. Amer. Math. Soc.},
  %FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {50},
      YEAR = {1944},
     PAGES = {267--278},
      ISSN = {0002-9904},
  % MRCLASS = {20.0X},
 % MRNUMBER = {0009955 (5,228a)},
%MRREVIEWER = {I. Kaplansky},
}

\bib{Ber1}{article}{%MR716835,
    AUTHOR = {Berend, Daniel},
     TITLE = {Multi-invariant sets on tori},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {280},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {509--532},
      ISSN = {0002-9947},
   %  CODEN = {TAMTAM},
   %MRCLASS = {11K06 (11K55 28D10 54A15)},
  %MRNUMBER = {716835 (85b:11064)},
%MRREVIEWER = {G{\'e}rard Rauzy},
       DOI = {\href{http://dx.doi.org/10.2307/1999631}{10.2307/1999631}},
  %     URL = ,
}


\bib{Ber2}{article}{%MR760973,
    AUTHOR = {Berend, Daniel},
     TITLE = {Multi-invariant sets on compact abelian groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {286},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {505--535},
      ISSN = {0002-9947},
   %  CODEN = {TAMTAM},
   %MRCLASS = {22D40 (11J61 11J69)},
  %MRNUMBER = {760973 (86e:22009)},
%MRREVIEWER = {Justin Peters},
       DOI = {\href{http://dx.doi.org/10.2307/1999808}{10.2307/1999808}},
 %      URL = ,
}

\bib{BD}{article}{%MR0365157,
    AUTHOR = {Bunce, John W.},
    AUTHOR = {Deddens, James A.},
     TITLE = {A family of simple C*-algebras related to weighted shift operators},
   JOURNAL = {J. Funct. Anal.},
    VOLUME = {19},
      YEAR = {1975},
     PAGES = {13--24},
  % MRCLASS = {46LXX (47C10)},
 % MRNUMBER = {0365157 (51 \#1410)},
%MRREVIEWER = {R. G. Douglas},
}

\bib{Bla}{book} {%MR2188261,
    AUTHOR = {Blackadar, Bruce},
     TITLE = {Operator Algebras},
    SERIES = {Encyclopaedia of Mathematical Sciences},
    VOLUME = {122},
     % NOTE = {Theory of C*-Algebras and von Neumann Algebras, Operator Algebras and Non-commutative Geometry, III},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
     PAGES = {xx+517},
      ISBN = {978-3-540-28486-4; 3-540-28486-9},
  % MRCLASS = {46L05 (46L10 46L80)},
 % MRNUMBER = {2188261 (2006k:46082)},
%MRREVIEWER = {Paul Jolissaint},
}

\bib{BLS1}{article}{
	AUTHOR={Brownlowe, Nathan},
	AUTHOR={Larsen, Nadia S.},	
	AUTHOR={Stammeier, Nicolai},
	TITLE={On $C^*$-algebras associated to right LCM semigroups},
	NOTE={preprint, \href{http://arxiv.org/abs/1406.5725}{arxiv.org:1406.5725}},
}

\bib{BLS2}{article}{
	AUTHOR={Brownlowe, Nathan},
	AUTHOR={Larsen, Nadia S.},	
	AUTHOR={Stammeier, Nicolai},
	TITLE={Nica-Toeplitz algebras associated to algebraic dynamical systems},
	NOTE={preprint, in preparation},
}

\bib{BO}{book} {%MR2391387,
    AUTHOR = {Brown, Nathanial P.},
    AUTHOR = {Ozawa, Narutaka},
     TITLE = {C*-Algebras and Finite-Dimensional Approximations},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {88},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {2008},
     PAGES = {xvi+509},
      ISBN = {978-0-8218-4381-9; 0-8218-4381-8}
  % MRCLASS = {46L05 (43A07 46-02 46L10)},
 % MRNUMBER = {2391387 (2009h:46101)},
%MRREVIEWER = {Mikael R{\o}rdam},
}

\bib{BOFS}{article}{
	AUTHOR = {Brown, Jonathan H.},
  AUTHOR = {Orloff Clark, Lisa},
	AUTHOR = {Farthing, Cynthia},
  AUTHOR = {Sims, Aidan},
  TITLE = {Simplicity of algebras associated to \'{e}tale groupoids},
  JOURNAL = {Semigroup Forum},
%  FJOURNAL = {Semigroup Forum},
    VOLUME = {88},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {433--452},
      ISSN = {0037-1912},
 %  MRCLASS = {Preliminary Data},
%  MRNUMBER = {3189105},
       DOI = {\href{http://dx.doi.org/10.1007/s00233-013-9546-z}{10.1007/s00233-013-9546-z}},
}

\bib{Car}{article} {%MR2772352,
    AUTHOR = {Carri{\'o}n, Jos{\'e} R.},
     TITLE = {Classification of a class of crossed product C*-algebras associated with residually finite groups},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {260},
      YEAR = {2011},
    NUMBER = {9},
     PAGES = {2815--2825},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L55 (20E26 46L80)},
%  MRNUMBER = {2772352 (2012e:46146)},
%MRREVIEWER = {Nadia S. Larsen},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2011.02.002}{10.1016/j.jfa.2011.02.002}},
}

\bib{CEL}{article}{
	AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Echterhoff, Siegfried},
    AUTHOR = {Li, Xin},
     TITLE = {On the $K$-theory of the C*-algebra generated by the left regular representation of an Ore semigroup}, %{$K$}
     JOURNAL = {to appear in J. Eur. Math. Soc.}
      YEAR = {2014},
       NOTE = {available as \href{http://arxiv.org/abs/1201.4680}{arxiv:1201.4680}},
}	

\bib{CEL2}{article}{%MR3094498,
AUTHOR = {Cuntz, Joachim},
AUTHOR = {Echterhoff, Siegfried},
AUTHOR = {Li, Xin},
TITLE = {On the $K$-theory of crossed products by automorphic semigroup actions}, %{$K$}
JOURNAL = {Q. J. Math.},
%FJOURNAL = {The Quarterly Journal of Mathematics},
VOLUME = {64},
YEAR = {2013},
NUMBER = {3},
     PAGES = {747--784},
      ISSN = {0033-5606},
   %MRCLASS = {19Dxx},
  %MRNUMBER = {3094498},
       DOI = {\href{http://dx.doi.org/10.1093/qmath/hat021}{10.1093/qmath/hat021}},
}	

\bib{CK}{article} {%MR561974,
    AUTHOR = {Cuntz, Joachim}, 
    AUTHOR = {Krieger, Wolfgang},
     TITLE = {A class of C*-algebras and topological {M}arkov chains},
   JOURNAL = {Invent. Math.},
  %FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {56},
      YEAR = {1980},
    NUMBER = {3},
     PAGES = {251--268},
      ISSN = {0020-9910},
     %CODEN = {INVMBH},
   %MRCLASS = {46L55 (54H20 58G10)},
  %MRNUMBER = {561974 (82f:46073a)},
%MRREVIEWER = {R. J. Nagel},
       DOI = {\href{http://dx.doi.org/10.1007/BF01390048}{10.1007/BF01390048}},
}

\bib{CL}{incollection}{%MR2732050,
    AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Li, Xin},
     TITLE = {The regular C*-algebra of an integral domain},
 BOOKTITLE = {Quanta of maths},
    SERIES = {Clay Math. Proc.},
    VOLUME = {11},
     PAGES = {149--170},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2010},
  % MRCLASS = {46L55 (11M55 11R04 46L05)},
 % MRNUMBER = {2732050 (2012c:46173)},
%MRREVIEWER = {Bora Yalkinoglu},
}

\bib{CLSV}{article} {%MR2837016,
    AUTHOR = {Carlsen, Toke Meier},
    AUTHOR = {Larsen, Nadia S.},
    AUTHOR = {Sims, Aidan},
    AUTHOR = {Vittadello, Sean T.},
     TITLE = {Co-universal algebras associated to product systems, and gauge-invariant uniqueness theorems},
   JOURNAL = {Proc. Lond. Math. Soc. (3)},
%  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {103},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {563--600},
      ISSN = {0024-6115},
%   MRCLASS = {46L05},
%  MRNUMBER = {2837016 (2012h:46085)},
%MRREVIEWER = {Yangping Jing},
       DOI = {\href{http://dx.doi.org/10.1112/plms/pdq028}{10.1112/plms/pdq028}},
}

\bib{CS}{article} {%MR2563500,
    AUTHOR = {Carlsen, Toke Meier},
    AUTHOR = {Silvestrov, Sergei},
     TITLE = {On the {E}xel crossed product of topological covering maps},
   JOURNAL = {Acta Appl. Math.},
%  FJOURNAL = {Acta Applicandae Mathematicae. An International Survey Journal
%              on Applying Mathematics and Mathematical Applications},
    VOLUME = {108},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {573--583},
      ISSN = {0167-8019},
%     CODEN = {AAMADV},
%   MRCLASS = {46L55 (37B05)},
%  MRNUMBER = {2563500 (2010k:46071)},
%MRREVIEWER = {Masaharu Kusuda},
       DOI = {\href{http://dx.doi.org/10.1007/s10440-008-9372-6}{10.1007/s10440-008-9372-6}},
}

\bib{Cun}{article}{%MR0467330,
    AUTHOR = {Cuntz, Joachim},
     TITLE = {Simple C*-algebras generated by isometries},
   JOURNAL = {Comm. Math. Phys.},
%  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {57},
      YEAR = {1977},
    NUMBER = {2},
     PAGES = {173--185},
      ISSN = {0010-3616},
%   MRCLASS = {46L05},
%  MRNUMBER = {0467330 (57 \#7189)},
%MRREVIEWER = {E. Stormer},
}

\bib{CV}{article}{
		AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Vershik, Anatoly},
     TITLE = {C*-algebras associated with endomorphisms and polymorphisms of compact abelian groups},
      YEAR = {2013},
issn={0010-3616},
journal={Comm. Math. Phys.},
volume={321},
number={1},
doi= {\href{http://dx.doi.org/10.1007/s00220-012-1647-0}{10.1007/s00220-012-1647-0}},
publisher={Springer-Verlag},
pages={157-179},
%language={English}
}	

\bib{DE}{book}{%MR2457798,
    AUTHOR = {Deitmar, Anton},
    AUTHOR = {Echterhoff, Siegfried},
     TITLE = {Principles of Harmonic Analysis},
    SERIES = {Universitext},
 PUBLISHER = {Springer, New York},
      YEAR = {2009},
     PAGES = {xvi+333},
      ISBN = {978-0-387-85468-7},
  % MRCLASS = {43-01 (22Dxx 22E30 46J10 46L05)},
 % MRNUMBER = {2457798 (2010g:43001)},
%MRREVIEWER = {Krishnan Parthasarathy},
}

\bib{DFK}{article}{
 	AUTHOR 	= {Davidson, Kenneth R.},
    AUTHOR 	= {Fuller, Adam H.},
    AUTHOR 	= {Kakariadis, Evgenios T.A.},
    TITLE	= {Semicrossed products of operator algebras by semigroups},
    %JOURNAL = {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/abs/1404.1906v1}{arxiv:1404.1906v1}}, 
}

\bib{dJST}{article}{%MR2913686,
    AUTHOR = {de Jeu, Marcel},
    AUTHOR = {Svensson, Christian},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {On the {B}anach {$\ast$}-algebra crossed product associated with a topological dynamical system},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {11},
     PAGES = {4746--4765},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46H99 54H20)},
 % MRNUMBER = {2913686},
%MRREVIEWER = {Claire Anantharaman-Delaroche},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2012.03.013}{10.1016/j.jfa.2012.03.013}},
       %URL = ,
}

\bib{dlH}{book}{%MR1786869,
    AUTHOR = {de la Harpe, Pierre},
     TITLE = {Topics in Geometric Group Theory},
    SERIES = {Chicago Lectures in Mathematics},
 PUBLISHER = {University of Chicago Press, Chicago, IL},
      YEAR = {2000},
     PAGES = {vi+310},
      ISBN = {0-226-31719-6; 0-226-31721-8},
  % MRCLASS = {20F65 (20F69 57M07)},
 % MRNUMBER = {1786869 (2001i:20081)},
%MRREVIEWER = {Lee Mosher},
}

\bib{EF}{article}{%MR2586349,
    AUTHOR = {Einsiedler, Manfred},
    AUTHOR = {Fish, Alexander},
     TITLE = {Rigidity of measures invariant under the action of a multiplicative semigroup of polynomial growth on $\IT$},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {151--157},
      ISSN = {0143-3857},
 %  MRCLASS = {37A10 (28D10 37A25)},
 % MRNUMBER = {2586349 (2011a:37005)},
%MRREVIEWER = {A. I. Danilenko},
       DOI = {\href{http://dx.doi.org/10.1017/S014338570800103X}{10.1017/S014338570800103X}},
}

\bib{EK}{article}{%MR2191228,
    AUTHOR = {Einsiedler, Manfred},
    AUTHOR = {Katok, Anatole},
     TITLE = {Rigidity of measures---the high entropy case and non-commuting foliations},
 %     NOTE = {Probability in mathematics},
   JOURNAL = {Israel J. Math.},
%  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {148},
      YEAR = {2005},
     PAGES = {169--238},
      ISSN = {0021-2172},
 %    CODEN = {ISJMAP},
 %  MRCLASS = {37C85 (37A15 37C40 37D30)},
 % MRNUMBER = {2191228 (2007d:37034)},
%MRREVIEWER = {S. G. Dani},
       DOI = {\href{http://dx.doi.org/10.1007/BF02775436}{10.1007/BF02775436}},
%       URL = ,
}

\bib{ER2}{article}{%MR2162134,
    AUTHOR = {Endimioni, G{\'e}rard},
    AUTHOR = {Robinson, Derek J. S.},
     TITLE = {On co-{H}opfian groups},
   JOURNAL = {Publ. Math. Debrecen},
 % FJOURNAL = {Publicationes Mathematicae Debrecen},
    VOLUME = {67},
      YEAR = {2005},
    NUMBER = {3-4},
     PAGES = {423--436},
      ISSN = {0033-3883},
   %  CODEN = {PUMAAR},
  % MRCLASS = {20F99},
 % MRNUMBER = {2162134 (2006e:20082)},
%MRREVIEWER = {Javier Otal},
}

\bib{Exe1}{article} {%MR2032486,
    AUTHOR = {Exel, Ruy},
     TITLE = {A new look at the crossed-product of a C*-algebra by an endomorphism},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {23},
      YEAR = {2003},
    NUMBER = {6},
     PAGES = {1733--1750},
      ISSN = {0143-3857},
  % MRCLASS = {46L55 (37B10)},
 % MRNUMBER = {2032486 (2004k:46119)},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385702001797}{10.1017/S0143385702001797}},
}

\bib{Exe2}{article}{%MR1966826,
    AUTHOR = {Exel, Ruy},
     TITLE = {Crossed-products by finite index endomorphisms and {KMS} states},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {199},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {153--188},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46L30)},
 % MRNUMBER = {1966826 (2004b:46094)},
%MRREVIEWER = {Masaharu Kusuda},
       DOI = {\href{http://dx.doi.org/10.1016/S0022-1236(02)00023-X}{10.1016/S0022-1236(02)00023-X}},
}

\bib{EaHR}{article} {%MR2985865,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {an Huef, Astrid},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Purely infinite simple {$C^*$}-algebras associated to integer dilation matrices},
   JOURNAL = {Indiana Univ. Math. J.},
 % FJOURNAL = {Indiana University Mathematics Journal},
    VOLUME = {60},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {1033--1058},
      ISSN = {0022-2518},
%     CODEN = {IUMJAB},
 %  MRCLASS = {46L05 (46L55)},
  %MRNUMBER = {2985865},
%MRREVIEWER = {Xin Li},
       DOI = {\href{http://dx.doi.org/10.1512/iumj.2011.60.4331}{10.1512/iumj.2011.60.4331}},
       %URL = ,
}

\bib{ER}{article}{%MR2371594,
    AUTHOR = {Exel, Ruy}, 
    AUTHOR = {Renault, Jean},
     TITLE = {Semigroups of local homeomorphisms and interaction groups},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {27},
      YEAR = {2007},
    NUMBER = {6},
     PAGES = {1737--1771},
      ISSN = {0143-3857},
  % MRCLASS = {46L55 (37B05 46L05)},
 % MRNUMBER = {2371594 (2009k:46124)},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385707000193}{10.1017/S0143385707000193}},
}	

\bib{EV}{article} {%MR2195591,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {Vershik, Anatoly},
     TITLE = {C*-algebras of irreversible dynamical systems},
   JOURNAL = {Canad. J. Math.},
%  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
%              Math\'ematiques},
    VOLUME = {58},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {39--63},
      ISSN = {0008-414X},
%     CODEN = {CJMAAB},
%   MRCLASS = {46L55 (37A55 46L05)},
%  MRNUMBER = {2195591 (2007d:46058)},
%MRREVIEWER = {Fr{\'e}d{\'e}ric Latr{\'e}moli{\`e}re},
       DOI = {\href{http://dx.doi.org/10.4153/CJM-2006-003-x}{10.4153/CJM-2006-003-x}},
}


\bib{Fur}{article} {%MR0213508,
    AUTHOR = {Furstenberg, Hillel},
     TITLE = {Disjointness in ergodic theory, minimal sets, and a problem in {D}iophantine approximation},
   JOURNAL = {Math. Systems Theory},
  %FJOURNAL = {Mathematical Systems Theory. An International Journal on
%              Mathematical Computing Theory},
    VOLUME = {1},
      YEAR = {1967},
     PAGES = {1--49},
      ISSN = {0025-5661},
   %MRCLASS = {28.70 (10.00)},
 % MRNUMBER = {0213508 (35 \#4369)},
%MRREVIEWER = {W. Parry}
}

\bib{Fow1}{article} {%MR1715181,
    AUTHOR = {Fowler, Neal J.},
    TITLE = {Compactly-aligned discrete product systems, and generalization of $\CO_{\infty}$},
   JOURNAL = {Internat. J. Math.},
  %FJOURNAL = {International Journal of Mathematics},
    VOLUME = {10},
      YEAR = {1999},
    NUMBER = {6},
     PAGES = {721--738},
      ISSN = {0129-167X},
  % MRCLASS = {46L05},
 % MRNUMBER = {1715181 (2002f:46104)},
       DOI = {\href{http://dx.doi.org/10.1142/S0129167X99000306}{10.1142/S0129167X99000306}},
}

\bib{Fow2}{article} {%MR1907896,
    AUTHOR = {Fowler, Neal J.},
     TITLE = {Discrete product systems of {H}ilbert bimodules},
   JOURNAL = {Pacific J. Math.},
 % FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {204},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {335--375},
      ISSN = {0030-8730},
%     CODEN = {PJMAAI},
%   MRCLASS = {46L08},
%  MRNUMBER = {1907896 (2003g:46070)},
%MRREVIEWER = {Arup Kumar Pal},
       DOI = {\href{http://dx.doi.org/10.2140/pjm.2002.204.335}{10.2140/pjm.2002.204.335}},
}

\bib{FPW}{article}{%MR3085824,
    AUTHOR = {Farthing, Cynthia},
    AUTHOR = {Patani, Nura},
    AUTHOR = {Willis, Paulette N.},
     TITLE = {The crossed-product structure of C*-algebras arising from topological dynamical systems},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {70},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {191--210},
      ISSN = {0379-4024},
   %MRCLASS = {46L55 (37A55)},
  %MRNUMBER = {3085824},
       DOI = {\href{http://dx.doi.org/10.7900/jot.2011may31.1924}{10.7900/jot.2011may31.1924}},
}

%\bib{Ga}{book} {%MR0107648,
 %   AUTHOR = {Gantmacher, F. R.},
  %   TITLE = {Applications of the theory of matrices},
  %  SERIES = {Translated by J. L. Brenner, with the assistance of D. W.
 %             Bushaw and S. Evanusa},
 %PUBLISHER = {Interscience Publishers, Inc., New York},
  %    YEAR = {1959},
  %   PAGES = {ix+317}
  % MRCLASS = {15.00 (65.00)},
 % MRNUMBER = {0107648 (21 \#6372b)},
%}

\bib{GG}{incollection}{%MR2962880,
    AUTHOR = {Goldsmith, Brendan},
    AUTHOR = {Gong, Ketao},
     TITLE = {A note on {H}opfian and co-{H}opfian abelian groups},
 BOOKTITLE = {Groups and Model Theory},
    SERIES = {Contemp. Math.},
    VOLUME = {576},
     PAGES = {129--136},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2012},
  % MRCLASS = {20K30 (20K21)},
 % MRNUMBER = {2962880},
%MRREVIEWER = {Simion Sorin P. Breaz},
       DOI = {\href{http://dx.doi.org/10.1090/conm/576/11356}{10.1090/conm/576/11356}},
}

\bib{Hed}{article}{%MR0259881,
    AUTHOR = {Hedlund, Gustav A.},
     TITLE = {Endomorphisms and automorphisms of the shift dynamical system},
   JOURNAL = {Math. Systems Theory},
%  FJOURNAL = {Mathematical Systems Theory. An International Journal on Mathematical Computing Theory},
    VOLUME = {3},
      YEAR = {1969},
     PAGES = {320--375},
      ISSN = {0025-5661},
  % MRCLASS = {54.82},
 % MRNUMBER = {0259881 (41 \#4510)},
%MRREVIEWER = {W. R. Utz},
}

\bib{Hir}{article} {%MR1896827,
    AUTHOR = {Hirshberg, Ilan},
     TITLE = {On C*-algebras associated to certain endomorphisms of discrete groups},
   JOURNAL = {New York J. Math.},
  %FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {99--109 (electronic)},
      ISSN = {1076-9803},
  % MRCLASS = {46L55},
 % MRNUMBER = {1896827 (2003d:46090)},
%MRREVIEWER = {Sriwulan Adji},
       NOTE = {\href{http://nyjm.albany.edu:8000/j/2002/8_99.html}{$nyjm.albany.edu:8000/j/2002/8_99$}},
}

\bib{HLS}{article}{
AUTHOR = {Hong, Jeong Hee},
AUTHOR = {Larsen, Nadia S.},
AUTHOR = {Szyma\'{n}ski, Wojciech},
TITLE  = {KMS states on Nica-Toeplitz algebras of product systems},
journal = {Internat. J. Math.},
volume = {23},
number = {12},
pages = {1250123},
year = {2012},
doi = {\href{http://www.worldscientific.com/doi/abs/10.1142/S0129167X12501236}{10.1142/S0129167X12501236}},
%eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0129167X12501236}
}

\bib{JT}{book} {%MR1124848,
    AUTHOR = {Knudsen Jensen, Kjeld},
    AUTHOR = {Thomsen, Klaus},
     TITLE = {Elements of {$KK$}-Theory},
    SERIES = {Mathematics: Theory \& Applications},
 PUBLISHER = {Birkh\"auser Boston Inc.},
   ADDRESS = {Boston, MA},
      YEAR = {1991},
     PAGES = {viii+202},
      ISBN = {0-8176-3496-7},
  % MRCLASS = {19K35 (46L80)},
 % MRNUMBER = {1124848 (94b:19008)},
%MRREVIEWER = {Jeffrey Fox},
       DOI = {\href{http://dx.doi.org/10.1007/978-1-4612-0449-7}{10.1007/978-1-4612-0449-7}},
}

\bib{Kat}{article} {%MR2067120,
    AUTHOR = {Katsura, Takeshi},
     TITLE = {A class of C*-algebras generalizing both graph algebras and homeomorphism C*-algebras. {I}. {F}undamental results},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {356},
      YEAR = {2004},
    NUMBER = {11},
     PAGES = {4287--4322 (electronic)},
      ISSN = {0002-9947},
    % CODEN = {TAMTAM},
   %MRCLASS = {46L05 (37B99 46L55 46L80)},
 %MRNUMBER = {2067120 (2005b:46119)},
%MRREVIEWER = {Valentin Deaconu},
       DOI = {\href{http://dx.doi.org/10.1090/S0002-9947-04-03636-0}{10.1090/S0002-9947-04-03636-0}},
}

\bib{Kir}{article}{
	AUTHOR 	= {Kirchberg, Eberhard},
	TITLE	= {The classication of purely infinite C*-algebras using Kasparov's theory},
	JOURNAL = {in Fields Inst. Commun, Amer. Math. Soc. Providence, to appear},
}

\bib{KK}{article}{
	AUTHOR = {Kalantar, Mehrdad},
	AUTHOR = {Kennedy, Matthew},
	TITLE  = {Boundaries of reduced C*-algebras of discrete groups},
	%JOURNAL = {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/pdf/1405.4359v1}{arxiv:1405.4359v1}},
}

%\bib{KP}{article} {%MR1745529,
 %   AUTHOR = {Kumjian, Alex},
  %  AUTHOR = {Pask, David},
   %  TITLE = {Higher rank graph C*-algebras},
   %JOURNAL = {New York J. Math.},
  %FJOURNAL = {New York Journal of Mathematics},
    %VOLUME = {6},
     % YEAR = {2000},
     %PAGES = {1--20 (electronic)},
     % ISSN = {1076-9803},
   %MRCLASS = {46L35 (46L45)},
  %MRNUMBER = {1745529 (2001b:46102)},
%MRREVIEWER = {Michael Frank},
      % URL = {http://nyjm.albany.edu:8000/j/2000/6_1.html}
%}

%\bib{KPRR}{article} {%MR1432596,
 %   AUTHOR = {Kumjian, Alex},
 %   AUTHOR = {Pask, David},
 %   AUTHOR = {Raeburn, Iain},
 %   AUTHOR = {Renault, Jean},
 %    TITLE = {Graphs, groupoids, and {C}untz-{K}rieger algebras},
 %  JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
 %   VOLUME = {144},
 %     YEAR = {1997},
 %   NUMBER = {2},
 %    PAGES = {505--541},
 %     ISSN = {0022-1236},
    % CODEN = {JFUAAW},
  % MRCLASS = {46L05 (46L55)},
 % MRNUMBER = {1432596 (98g:46083)},
%MRREVIEWER = {Masatoshi Enomoto},
  %     DOI = {10.1006/jfan.1996.3001},
  %     URL = {http://dx.doi.org/10.1006/jfan.1996.3001},
%}

\bib{Kri}{article} {%MR1934386,
    AUTHOR = {Kribs, David W.},
     TITLE = {Inductive limit algebras from periodic weighted shifts on {F}ock space},
   JOURNAL = {New York J. Math.},
%  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {145--159 (electronic)},
      ISSN = {1076-9803},
%   MRCLASS = {46L05 (46L35)},
%  MRNUMBER = {1934386 (2004b:46073)},
%MRREVIEWER = {Il Bong Jung},
       NOTE = {\href{http://nyjm.albany.edu:8000/j/2002/8_145.html}{nyjm.albany.edu:8000/j/2002/8_145}},
}

\bib{KT}{article}{%MR1088230,
    AUTHOR = {Kawamura, Shinz{\=o}},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {Properties of topological dynamical systems and corresponding {$C^*$}-algebras},
   JOURNAL = {Tokyo J. Math.},
%  FJOURNAL = {Tokyo Journal of Mathematics},
    VOLUME = {13},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {251--257},
      ISSN = {0387-3870},
%   MRCLASS = {46L55 (54H20)},
%  MRNUMBER = {1088230 (92e:46131)},
%MRREVIEWER = {John Quigg},
       DOI = {\href{http://dx.doi.org/10.3836/tjm/1270132260}{10.3836/tjm/1270132260}},
 %      URL = ,
}

\bib{Lac}{article} {%MR1766113,
    AUTHOR = {Laca, Marcelo},
     TITLE = {From endomorphisms to automorphisms and back: dilations and full corners},
   JOURNAL = {J. London Math. Soc. (2)},
%  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {61},
      YEAR = {2000},
    NUMBER = {3},
     PAGES = {893--904},
      ISSN = {0024-6107},
%     CODEN = {JLMSAK},
%   MRCLASS = {46L55 (46L89)},
%  MRNUMBER = {1766113 (2002a:46094)},
       DOI = {\href{http://dx.doi.org/10.1112/S0024610799008492}{10.1112/S0024610799008492}},
}

\bib{Lan}{book}{%MR1325694,
    AUTHOR = {Lance, Christopher E.},
     TITLE = {Hilbert C*-Modules},
    SERIES = {London Mathematical Society Lecture Note Series},
    VOLUME = {210},
   %   NOTE = {A Toolkit for Operator Algebraists},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1995},
     PAGES = {x+130},
      ISBN = {0-521-47910-X},
  % MRCLASS = {46L05 (46H25 46K05 46L80 46M05 47D25)},
 % MRNUMBER = {1325694 (96k:46100)},
%MRREVIEWER = {Robert S. Doran},
       DOI = {\href{http://dx.doi.org/10.1017/CBO9780511526206}{10.1017/CBO9780511526206}},
}

\bib{Lar}{article} {%MR2669415,
    AUTHOR = {Larsen, Nadia S.},
     TITLE = {Crossed products by abelian semigroups via transfer operators},
   JOURNAL = {Ergodic Theory Dynam. Systems},
%  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {1147--1164},
      ISSN = {0143-3857},
%   MRCLASS = {46L55},
%  MRNUMBER = {2669415 (2011j:46114)},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385709000509}{10.1017/S0143385709000509}},
}

\bib{LR2}{article}{%MR1402771,
    AUTHOR = {Laca, Marcelo},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Semigroup crossed products and the {T}oeplitz algebras of nonabelian groups},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {139},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {415--440},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46L35 47B35)},
 % MRNUMBER = {1402771 (97h:46109)},
%MRREVIEWER = {Erik B{\'e}dos},
       DOI = {\href{http://dx.doi.org/10.1006/jfan.1996.0091}{10.1006/jfan.1996.0091}},
}

\bib{LR}{article} {%MR2339372,
    AUTHOR = {Larsen, Nadia S.},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Projective multi-resolution analyses arising from direct limits of {H}ilbert modules},
   JOURNAL = {Math. Scand.},
%  FJOURNAL = {Mathematica Scandinavica},
    VOLUME = {100},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {317--360},
      ISSN = {0025-5521},
%     CODEN = {MTSCAN},
%   MRCLASS = {42C40 (28A80 46C05 46H25 46L08 60D05)},
%  MRNUMBER = {2339372 (2008m:42059)},
%MRREVIEWER = {Palle E. T. Jorgensen},
}

\bib{Li0}{article}{%MR2721644,
    AUTHOR = {Li, Xin},
     TITLE = {Ring C*-algebras},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {348},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {859--898},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L05 (11R56 16D30 58B34)},
 % MRNUMBER = {2721644 (2012a:46100)},
%MRREVIEWER = {Nadia S. Larsen},
       DOI = {\href{http://dx.doi.org/10.1007/s00208-010-0502-x}{10.1007/s00208-010-0502-x}},
}

\bib{Li1}{article} {%MR2900468,
    AUTHOR = {Li, Xin},
     TITLE = {Semigroup C*-algebras and amenability of semigroups},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {10},
     PAGES = {4302--4340},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L05},
%  MRNUMBER = {2900468},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2012.02.020}{10.1016/j.jfa.2012.02.020}},
}

\bib{Li2}{article}{%MR3077884,
    AUTHOR = {Li, Xin},
     TITLE = {Nuclearity of semigroup C*-algebras and the connection to amenability},
   JOURNAL = {Adv. Math.},
%  FJOURNAL = {Advances in Mathematics},
    VOLUME = {244},
      YEAR = {2013},
     PAGES = {626--662},
      ISSN = {0001-8708},
%   MRCLASS = {46L05 (20M12 43A07)},
%  MRNUMBER = {3077884},
%MRREVIEWER = {Takahiro Sudo},
       DOI = {\href{http://dx.doi.org/10.1016/j.aim.2013.05.016}{10.1016/j.aim.2013.05.016}},
}

\bib{Lin}{article}{%MR1814969,
    AUTHOR = {Lin, Huaxin},
     TITLE = {Classification of simple tracially {AF} C*-algebras},
   JOURNAL = {Canad. J. Math.},
%  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de Math\'{e}matiques},
    VOLUME = {53},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {161--194},
      ISSN = {0008-414X},
   %  CODEN = {CJMAAB},
  % MRCLASS = {46L35 (19K14 46L05 46L80)},
 % MRNUMBER = {1814969 (2002h:46102)},
%MRREVIEWER = {Judith A. Packer},
       DOI = {\href{http://dx.doi.org/10.4153/CJM-2001-007-8}{10.4153/CJM-2001-007-8}},
}

\bib{LS}{incollection} {%MR1928527,
    AUTHOR = {Lind, Douglas},
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Symbolic and algebraic dynamical systems},
 BOOKTITLE = {Handbook of dynamical systems, {V}ol.\ 1{A}},
     PAGES = {765--812},
 PUBLISHER = {North-Holland, Amsterdam},
      YEAR = {2002},
   %MRCLASS = {37B50 (37A15 37B10)},
  %MRNUMBER = {1928527 (2003h:37017)},
%MRREVIEWER = {Anthony Quas},
       DOI = {\href{http://dx.doi.org/10.1016/S1874-575X(02)80012-1}{10.1016/S1874-575X(02)80012-1}},
 %      URL = ,
}

\bib{Mat}{article} {%MR1774695,
    AUTHOR = {Matsumoto, Kengo},
     TITLE = {On automorphisms of C*-algebras associated with subshifts},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {44},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {91--112},
      ISSN = {0379-4024}
  % MRCLASS = {46L55 (37A55 37B10)},
 % MRNUMBER = {1774695 (2001g:46147)},
%MRREVIEWER = {A. I. Danilenko},
}

\bib{MS}{article}{
	AUTHOR 	= {Matui, Hiroki},
	AUTHOR 	= {Sato, Yasuhiko},
	TITLE 	= {Decomposition rank of UHF-absorbing C*-algebras},
	JOURNAL	= {to appear in Duke Math. J.},
	Note	= {available as \href{http://arxiv.org/abs/1303.4371v2}{arxiv:1303.4371v2}},
}

\bib{MW}{article}{
	AUTHOR 	= {Maloney, Ben},
	AUTHOR 	= {Willis, Paulette N.},
	TITLE 	= {Examples of $*$-commuting maps},
	%JOURNAL	= {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/abs/1101.3795v2}{arxiv:1101.3795v2}},	
}

\bib{Muc}{article}{%MR2136018,
    AUTHOR = {Muchnik, Roman},
     TITLE = {Semigroup actions on $\IT^n$},
   JOURNAL = {Geom. Dedicata},
  %FJOURNAL = {Geometriae Dedicata},
    VOLUME = {110},
      YEAR = {2005},
     PAGES = {1--47},
      ISSN = {0046-5755},
   %  CODEN = {GEMDAT},
  % MRCLASS = {37B05 (20M20)},
 % MRNUMBER = {2136018 (2006i:37022)},
%MRREVIEWER = {Daniel Berend},
}

\bib{Nic}{article}{%MR1241114,
    AUTHOR = {Nica, Alexandru},
     TITLE = {C*-algebras generated by isometries and {W}iener-{H}opf operators},
   JOURNAL = {J. Operator Theory},
 % FJOURNAL = {Journal of Operator Theory},
    VOLUME = {27},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {17--52},
      ISSN = {0379-4024},
  % MRCLASS = {46L35 (47B35 47C10)},
 % MRNUMBER = {1241114 (94m:46094)},
%MRREVIEWER = {Ra{\'u}l E. Curto},
}


\bib{NS}{book} {%MR2251116,				%%%notwendig? Walters als Referenz!
    AUTHOR = {Neshveyev, Sergey},
    AUTHOR = {St{\o}rmer, Erling},
     TITLE = {Dynamical Entropy in Operator Algebras},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A Series of Modern Surveys in Mathematics [Results in Mathematics and Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
    VOLUME = {50},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
     PAGES = {x+296},
      ISBN = {978-3-540-34670-8; 3-540-34670-8}
   %MRCLASS = {46L55 (28D20 37B40 46L54 82C10)},
  %MRNUMBER = {2251116 (2007m:46108)},
%MRREVIEWER = {Adam G. Skalski}
}

\bib{Orf}{article} {%MR2550195,
    AUTHOR = {Orfanos, Stefanos},
     TITLE = {Generalized {B}unce-{D}eddens algebras},
   JOURNAL = {Proc. Amer. Math. Soc.},
%  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {138},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {299--308},
      ISSN = {0002-9939},
%     CODEN = {PAMYAR},
%   MRCLASS = {46L55 (46L05 47L65)},
%  MRNUMBER = {2550195 (2011a:46104)},
%MRREVIEWER = {Michal Zajac},
       DOI = {\href{http://dx.doi.org/10.1090/S0002-9939-09-10071-0}{10.1090/S0002-9939-09-10071-0}},
}

\bib{Oza}{article}{%MR1763912,
    AUTHOR = {Ozawa, Narutaka},
     TITLE = {Amenable actions and exactness for discrete groups},
   JOURNAL = {C. R. Acad. Sci. Paris S\'{e}r. I Math.},
%  FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.Math\'ematique},
    VOLUME = {330},
      YEAR = {2000},
    NUMBER = {8},
     PAGES = {691--695},
      ISSN = {0764-4442},
   %  CODEN = {CASMEI},
  % MRCLASS = {22D25 (43A35 46L06 46L55)},
 % MRNUMBER = {1763912 (2001g:22007)},
%MRREVIEWER = {Alain Valette},
       DOI = {\href{http://dx.doi.org/10.1016/S0764-4442(00)00248-2}{10.1016/S0764-4442(00)00248-2}},
}

\bib{Par}{incollection}{%MR1411219,
    AUTHOR = {Parry, William},
     TITLE = {Squaring and cubing the circle \mdash {R}udolph's theorem},
 BOOKTITLE = {Ergodic theory of $\Z^d$-actions ({W}arwick,
              1993--1994)},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {228},
     PAGES = {177--183},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {1996},
  % MRCLASS = {28D15 (11K16)},
 % MRNUMBER = {1411219 (97h:28009)},
%MRREVIEWER = {Thomas Ward},
       DOI = {\href{http://dx.doi.org/10.1017/CBO9780511662812.006}{10.1017/CBO9780511662812.006}},
}

\bib{Phi}{article} {%MR1745197,
    AUTHOR = {Phillips, Christopher N.},
     TITLE = {A classification theorem for nuclear purely infinite simple C*-algebras},
   JOURNAL = {Doc. Math.},
  %FJOURNAL = {Documenta Mathematica},
    VOLUME = {5},
      YEAR = {2000},
     PAGES = {49--114 (electronic)},
      ISSN = {1431-0635},
 %  MRCLASS = {46L05 (19K56 46L35 46L80)},
  %MRNUMBER = {1745197 (2001d:46086b)},
%MRREVIEWER = {Mikael R{\o}rdam},
}

\bib{Pim}{incollection} {%MR1426840,
    AUTHOR = {Pimsner, Mihai V.},
     TITLE = {A class of C*-algebras generalizing both {C}untz-{K}rieger algebras and crossed products by $\Z$},
 BOOKTITLE = {Free probability theory ({W}aterloo, {ON}, 1995)},
    SERIES = {Fields Inst. Commun.},
    VOLUME = {12},
     PAGES = {189--212},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {1997},
  % MRCLASS = {46L05 (46L55 46L80)},
 % MRNUMBER = {1426840 (97k:46069)},
%MRREVIEWER = {Michael Frank},
}

\bib{PR}{article} {%MR1964302,
    AUTHOR = {Packer, Judith A.},
    AUTHOR = {Rieffel, Marc A.},
     TITLE = {Wavelet filter functions, the matrix completion problem, and modules over $C(\IT^n)$},
   JOURNAL = {J. Fourier Anal. Appl.},
  %FJOURNAL = {The Journal of Fourier Analysis and Applications},
    VOLUME = {9},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {101--116},
      ISSN = {1069-5869},
  % MRCLASS = {42C40 (46H25 46L99 94A12)},
 % MRNUMBER = {1964302 (2003m:42063)},
%MRREVIEWER = {Jo Ward},
       DOI = {\href{http://dx.doi.org/10.1007/s00041-003-0010-4}{10.1007/s00041-003-0010-4}},
}


%Referenz im Ausblick zu den Bereichen, die helfen könnten. 
%\bib{R}{book} {%MR584266,
 %   AUTHOR = {Renault, Jean},
 %    TITLE = {A groupoid approach to {$C\sp{\ast} $}-algebras},
 %   SERIES = {Lecture Notes in Mathematics},
 %   VOLUME = {793},
% PUBLISHER = {Springer},
%   ADDRESS = {Berlin},
%      YEAR = {1980},
%     PAGES = {ii+160},
%      ISBN = {3-540-09977-8},
  % MRCLASS = {46Lxx (22D25 22D40)},
  %MRNUMBER = {584266 (82h:46075)},
%MRREVIEWER = {A. K. Seda},
%}

\bib{Rud}{article} {%MR1062766,
    AUTHOR = {Rudolph, Daniel J.},
     TITLE = {{$\times 2$} and {$\times 3$} invariant measures and entropy},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  %FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {10},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {395--406},
      ISSN = {0143-3857},
  % MRCLASS = {28D20},
  %MRNUMBER = {1062766 (91g:28026)},
%MRREVIEWER = {Ladislav Andrey},
      DOI = {\href{http://dx.doi.org/10.1017/S0143385700005629}{10.1017/S0143385700005629}},
}

%\bib{RL}{book} {%MR1783408,
 %   AUTHOR = {R{\o}rdam, M.},
  %  AUTHOR = {Larsen, F.},
   % AUTHOR = {Laustsen, N.},
    % TITLE = {An introduction to {$K$}-theory for C*-algebras},
    %SERIES = {London Mathematical Society Student Texts},
    %VOLUME = {49},
 %PUBLISHER = {Cambridge University Press},
 %  ADDRESS = {Cambridge},
  %    YEAR = {2000},
   %  PAGES = {xii+242},
    %  ISBN = {0-521-78334-8; 0-521-78944-3}
  % MRCLASS = {46-01 (19K35 46L80)},
 % MRNUMBER = {1783408 (2001g:46001)},
%MRREVIEWER = {{\'E}ric Leichtnam},
%}


%\bib{RS}{article} {%MR1713322,
 %   AUTHOR = {Robertson, Guyan},
  %  AUTHOR = {Steger, Tim},
   %  TITLE = {Affine buildings, tiling systems and higher rank
    %          {C}untz-{K}rieger algebras},
   %JOURNAL = {J. Reine Angew. Math.},
  %FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
    %VOLUME = {513},
     % YEAR = {1999},
     %PAGES = {115--144},
     % ISSN = {0075-4102},
   %  CODEN = {JRMAA8},
  % MRCLASS = {46L05 (20E42 46L55)},
 % MRNUMBER = {1713322 (2000j:46109)},
%MRREVIEWER = {Claudia Pinzari},
      % DOI = {10.1515/crll.1999.057},
       %URL = {http://dx.doi.org/10.1515/crll.1999.057}
%}

\bib{Sch1}{book} {%MR3024809,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Dynamical systems of algebraic origin},
    SERIES = {Modern Birkh\"auser Classics},
%      NOTE = {[2011 reprint of the 1995 original]},% [MR1345152]},
 PUBLISHER = {Birkh\"auser/Springer Basel AG, Basel},
      YEAR = {1995},
     PAGES = {xviii+310},
      ISBN = {978-3-0348-0276-5; 978-3-0348-0277-2},
   %MRCLASS = {01A75},
 % MRNUMBER = {3024809},
}

\bib{Sch2}{incollection} {%MR1905342,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {The dynamics of algebraic {$\Z^d$}-actions},
 BOOKTITLE = {European {C}ongress of {M}athematics, {V}ol. {I} ({B}arcelona,
              2000)},
    SERIES = {Progr. Math.},
    VOLUME = {201},
     PAGES = {543--553},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {2001},
   %MRCLASS = {37A15 (28D20)},
  %MRNUMBER = {1905342 (2003e:37007)},
%MRREVIEWER = {Thomas Ward},
}

\bib{Sie}{article}{%MR2775364,
    AUTHOR = {Sierakowski, Adam},
     TITLE = {The ideal structure of reduced crossed products},
   JOURNAL = {M\"unster J. Math.},
  %FJOURNAL = {M\"unster Journal of Mathematics},
    VOLUME = {3},
      YEAR = {2010},
     PAGES = {237--261},
      ISSN = {1867-5778},
  % MRCLASS = {46L55 (22D25)},
 % MRNUMBER = {2775364 (2012g:46103)},
%MRREVIEWER = {Tomoyoshi Ohwada},
}


%\bib{Sim}{article} {%MR2270926,
 %   AUTHOR = {Sims, Aidan},
  %   TITLE = {Gauge-invariant ideals in the {$C\sp *$}-algebras of finitely
   %           aligned higher-rank graphs},
   %JOURNAL = {Canad. J. Math.},
  %FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
%              Math\'ematiques},
%    VOLUME = {58},
 %     YEAR = {2006},
  %  NUMBER = {6},
   %  PAGES = {1268--1290},
    %  ISSN = {0008-414X},
   %  CODEN = {CJMAAB},
   %MRCLASS = {46L05},
  %MRNUMBER = {2270926 (2007j:46095)},
%MRREVIEWER = {Bernhard Burgstaller},
     %  URL = {http://journals.cms.math.ca/ams/ams-redirect.php?Journal=CJM&Volume=58&FirstPage=1268}
%}

\bib{Schm}{incollection} {%MR2090771,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Algebraic $\Z^d$-actions on zero-dimensional compact abelian groups},
 BOOKTITLE = {Modern dynamical systems and applications},
     PAGES = {185--209},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2004},
  % MRCLASS = {37A15 (28D15 34A45 37A25 37A35)},
 % MRNUMBER = {2090771 (2005g:37003)},
%MRREVIEWER = {Manfred Einsiedler},
}

\bib{Sol}{article}{%MR2225464,
    AUTHOR = {Solel, Baruch},
     TITLE = {Representations of product systems over semigroups and dilations of commuting {CP} maps},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {235},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {593--618},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L08 (46L57 47A20)},
%  MRNUMBER = {2225464 (2007h:46073)},
%MRREVIEWER = {B. V. Rajarama Bhat},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2005.11.014}{10.1016/j.jfa.2005.11.014}},
}


\bib{Sta}{article}{%MR1200792,
    AUTHOR = {Stacey, Peter J.},
     TITLE = {Crossed products of C*-algebras by {$\ast$}-endomorphisms},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  %FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure Mathematics and Statistics},
    VOLUME = {54},
      YEAR = {1993},
    NUMBER = {2},
     PAGES = {204--212},
      ISSN = {0263-6115},
   %  CODEN = {JAMADS},
  % MRCLASS = {46L05 (46L55)},
 % MRNUMBER = {1200792 (94a:46077)},
%MRREVIEWER = {Shuang Zhang},
}

\bib{Sta1}{article}{
	AUTHOR={Stammeier, Nicolai},
	TITLE={On C*-algebras of irreversible algebraic dynamical systems},
	NOTE={preprint, \href{http://arxiv.org/abs/1411.2776}{arxiv:1411.2776}},
}

\bib{Sta2}{article}{
	AUTHOR={Stammeier, Nicolai},
	TITLE={Topological freeness for $*$-commuting covering maps},
	NOTE={preprint, \href{http://arxiv.org/abs/1311.0793}{arxiv:1311.0793}},
}

\bib{ST}{article}{%MR2498769,
    AUTHOR = {Svensson, Christian},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {On the commutant of {$C(X)$} in {$C^*$}-crossed products by {$\Z$} and their representations},
   JOURNAL = {J. Funct. Anal.},
  %FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {256},
      YEAR = {2009},
    NUMBER = {7},
     PAGES = {2367--2386},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55},
 % MRNUMBER = {2498769 (2010f:46105)},
%MRREVIEWER = {Steven P. Kaliszewski},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2009.02.002}{10.1016/j.jfa.2009.02.002}},
       %URL = ,
}

\bib{SY}{article} {%MR2718947,
    AUTHOR = {Sims, Aidan},
    AUTHOR = {Yeend, Trent},
     TITLE = {C*-algebras associated to product systems of {H}ilbert bimodules},
   JOURNAL = {J. Operator Theory},
%  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {64},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {349--376},
      ISSN = {0379-4024},
%   MRCLASS = {46L05 (46L08)},
%  MRNUMBER = {2718947 (2011j:46092)},
%MRREVIEWER = {Vladimir Manuilov},
}

%\bib{SZ}{article} {%MR2383707,
 %   AUTHOR = {Skalski, Adam},
  %  AUTHOR = {Zacharias, Joachim},
  %   TITLE = {Entropy of shifts on higher-rank graph {$C\sp *$}-algebras},
  % JOURNAL = {Houston J. Math.},
  %FJOURNAL = {Houston Journal of Mathematics},
   % VOLUME = {34},
    %  YEAR = {2008},
    %NUMBER = {1},
    % PAGES = {269--282},
    %  ISSN = {0362-1588},
    % CODEN = {HJMADZ},
   %MRCLASS = {46L55 (37B10 37B40)},
 % MRNUMBER = {2383707 (2009j:46165)},
%MRREVIEWER = {Aidan D. Sims}
%}

\bib{Tu}{article} {%MR1703305,
    AUTHOR = {Tu, Jean-Louis},
     TITLE = {La conjecture de {B}aum-{C}onnes pour les feuilletages moyennables},
   JOURNAL = {$K$-Theory},
 % FJOURNAL = {$K$-Theory. An Interdisciplinary Journal for the Development,
  %            Application, and Influence of $K$-Theory in the Mathematical
   %           Sciences},
    VOLUME = {17},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {215--264},
      ISSN = {0920-3036},
   %  CODEN = {KTHEEO},
  % MRCLASS = {19K35 (46L85 58J22)},
 % MRNUMBER = {1703305 (2000g:19004)},
%MRREVIEWER = {Hiroshi Takai},
       DOI = {\href{http://dx.doi.org/10.1023/A:1007744304422}{10.1023/A:1007744304422}},
}

\bib{Vie}{thesis}{
	AUTHOR = {Vieira, Felipe},
	TITLE  = {C*-algebras associated with endomorphisms of groups},
	SCHOOL = {University of M\"unster},
	YEAR   = {2013}, 
	NOTE    = {summary available as \href{http://arxiv.org/pdf/1308.1386v2}{arxiv:1308.1386v2}},
}

\bib{Wal}{book}{%MR648108,
    AUTHOR = {Walters, Peter},
     TITLE = {An Introduction to Ergodic Theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {79},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1982},
     PAGES = {ix+250},
      ISBN = {0-387-90599-5},
   %MRCLASS = {28Dxx (54H20 58F11)},
  %MRNUMBER = {648108 (84e:28017)},
%MRREVIEWER = {M. A. Akcoglu},
}

\bib{Wat}{article}{%MR996807,
    AUTHOR = {Watatani, Yasuo},
     TITLE = {Index for C*-subalgebras},
   JOURNAL = {Mem. Amer. Math. Soc.},
 % FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {83},
      YEAR = {1990},
    NUMBER = {424},
     PAGES = {vi+117},
      ISSN = {0065-9266},
   %  CODEN = {MAMCAU},
%   MRCLASS = {46L05 (19K14 46L40 46L80 46M20)},
 % MRNUMBER = {996807 (90i:46104)},
%MRREVIEWER = {Masatoshi Enomoto},
       DOI = {\href{http://dx.doi.org/10.1090/memo/0424}{10.1090/memo/0424}},
}

\bib{Wil}{book}{%MR2288954,
    AUTHOR = {Williams, Dana P.},
     TITLE = {Crossed Products of C*-Algebras},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {134},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2007},
     PAGES = {xvi+528},
      ISBN = {978-0-8218-4242-3; 0-8218-4242-0},
  % MRCLASS = {46-02 (22D25 46L05 46L35 46L55 46L85)},
 % MRNUMBER = {2288954 (2007m:46003)},
%MRREVIEWER = {Jonathan M. Rosenberg},
}

\bib{Wil2}{thesis} {%MR2941447,
    AUTHOR = {Willis, Paulette Nicole},
     TITLE = {C*-Algebras of labeled graphs and $*$-commuting endomorphisms},
      NOTE = {Thesis (Ph.D.)--The University of Iowa},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2010},
     PAGES = {113},
      ISBN = {978-1124-07016-2},
  % MRCLASS = {Thesis},
 % MRNUMBER = {2941447},
}

\bib{Win}{article}{%MR2179780,
    AUTHOR = {Winter, Wilhelm},
     TITLE = {On topologically finite-dimensional simple C*-algebras},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {332},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {843--878},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L85 (19K14 46L05 46L35)},
 % MRNUMBER = {2179780 (2006i:46102)},
%MRREVIEWER = {Huaxin Lin},
       DOI = {\href{http://dx.doi.org/10.1007/s00208-005-0657-z}{10.1007/s00208-005-0657-z}},
}

\bib{Yee}{article} {%MR2301938,
    AUTHOR = {Yeend, Trent},
     TITLE = {Groupoid models for the C*-algebras of topological higher-rank graphs},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {57},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {95--120},
      ISSN = {0379-4024},
  % MRCLASS = {46L05 (22D25 46L55)},
 % MRNUMBER = {2301938 (2008f:46074)},
}

\bib{Zel}{article} {%MR0241994,
    AUTHOR = {Zeller-Meier, Georges},
     TITLE = {Produits crois\'{e}s d'une C*-alg\`{e}bre par un groupe d'automorphismes},
   JOURNAL = {J. Math. Pures Appl. (9)},
%  FJOURNAL = {Journal de Math\'ematiques Pures et Appliqu\'ees. Neuvi\`eme
 %             S\'erie},
    VOLUME = {47},
      YEAR = {1968},
     PAGES = {101--239},
      ISSN = {0021-7824},
%   MRCLASS = {46.65},
%  MRNUMBER = {0241994 (39 \#3329)},
%MRREVIEWER = {B. Russo},
}

\end{biblist}
%\end{bibdiv}
